Time-Varying Gaussian Process Bandit Optimization

We consider the sequential Bayesian optimization problem with bandit feedback, adopting a formulation that allows for the reward function to vary with time. We model the reward function using a Gaussian process whose evolution obeys a simple Markov model. We introduce two natural extensions of the classical Gaussian process upper confidence bound (GP-UCB) algorithm. The first, R-GP-UCB, resets GP-UCB at regular intervals. The second, TV-GP-UCB, instead forgets about old data in a smooth fashion. Our main contribution comprises of novel regret bounds for these algorithms, providing an explicit characterization of the trade-off between the time horizon and the rate at which the function varies. We illustrate the performance of the algorithms on both synthetic and real data, and we find the gradual forgetting of TV-GP-UCB to perform favorably compared to the sharp resetting of R-GP-UCB. Moreover, both algorithms significantly outperform classical GP-UCB, since it treats stale and fresh data equally.

==> Time-Varying Gaussian Process Bandit Optimization/defns.tex <==
%dvips -Ppdf -tletter -G0 -o paper.ps paper.dvi

% define a box
\newcommand{\emptybox}[2]{%
  \vspace{.3in}
  \fbox{%
  \begin{minipage}{6in}%
  #2\hfill\vspace{#1in}%
  \end{minipage}}
  \vspace{.3in}
  }

% mycomment
\newcommand{\mycomment}[1]%
{\par {\bfseries \color{green} \scriptsize{#1} \par}}

% quiz
\newcommand{\quiz}[1]%
{\par {\bfseries \color{red} \scriptsize{Quiz: #1} \par}} 
% review
\newcommand{\review}[1]%
{\par {\bfseries \color{green} \scriptsize{#1} \par}}
% lab
\newcommand{\lab}[1]%
{\par {\bfseries \color{cyan} \scriptsize{#1} \par}}
% concept 
\newcommand{\concept}[1]%
{\emph{\textbf{\color{blue} #1}}}


%*********For chapter on binary and categorical data***********
\newcommand{\deriv}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\secondderiv}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}}
\newcommand\cut[1]{}
\newcommand{\llpl}{ logistic-log-partition }
\newcommand{\llplc}{ Logistic-Log-Partition }
\newcommand{\llps} {LLP}
\newcommand{\lse}{\mbox{lse}}
\newcommand{\llp}{\mbox{llp}}
\newcommand{\lvb}{\underline{f}}
\newcommand{\neglvb}{\overline{f}}
\newcommand{\primal}{f}
\newcommand{\lL}{g}
\newcommand{\lagrange}{\mathcal{L}}
\newcommand{\elbo}{\underline{\mathcal{L}}_n}
\newcommand{\elbofull}{\underline{\mathcal{L}}_n(\vtheta, \vgamma_n, \valpha_n)}
\newcommand{\elbofinal}{\underline{\mathcal{L}}}
\newcommand{\elbofinalfull}{\underline{\mathcal{L}}(\vtheta, \vgamma, \valpha)}
\newcommand{\bm}{\overline{m}}
\newcommand{\bv}{\overline{v}}
\newcommand{\bvm}{\overline{\vm}}
\newcommand{\bvv}{\overline{\vv}}
\newcommand{\bvV}{\overline{\vV}}

\newcommand{\tvx}{\widetilde{\vx}}
\newcommand{\tvX}{\widetilde{\vX}}
\newcommand{\tmu}{\widetilde{\vmu}}
\newcommand{\tSigma}{\widetilde{\vSigma}}
\newcommand{\tm}{\widetilde{m}}
\newcommand{\tv}{\widetilde{v}}
\newcommand{\tsigma}{\widetilde{\sigma}}
\newcommand{\tV}{\widetilde{V}}
\newcommand{\tvSigma}{\widetilde{\vSigma}}
\newcommand{\tg}{\widetilde{\gamma}}
\newcommand{\tvm}{\widetilde{\vm}}
\newcommand{\tvv}{\widetilde{\vv}}
\newcommand{\tvV}{\widetilde{\vV}}
\newcommand{\tvg}{\widetilde{\vgamma}}

\newcommand{\bO}{\mathbb{O}}
\newcommand{\mydefine}{:=}
\newcommand{\offset}[1]{\vw_{0#1}}
\newcommand{\loadMat}[1]{\vW_{#1}}
%\newcommand{\lse}{\mbox{llp}}
\usepackage{algorithm}



\def\Section {\S}
%allows you to replace the rather long "Section 5" by §5 when you use \Section 5. 

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }
 
%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}

%% a trick that makes the title take up less space for many style files (but not article)
%\addtolength{\titlebox}{-1.8cm}

%% densify spacing in bibliographies
\newcommand{\bibfix}{%    PUT \bibfix in file.bbl after first line
    \setlength{\parsep}{\parskip}%
    \setlength{\itemsep}{0cm}%
    \setlength{\topsep}{\parskip}%
    \setlength{\parskip}{0cm}%
    \setlength{\partopsep}{0cm}%
    \setlength{\listparindent}{\parindent}%
    \setlength{\labelwidth}{10pt}%
    \setlength{\labelsep}{0pt}%
    \setlength{\leftskip}{0pt}%
    \setlength{\leftmargin}{0pt}%
}

%% change margins
%\setlength{\textwidth}{7in}
%\setlength{\textheight}{8.75in}
%\setlength{\oddsidemargin}{-0.25in}
%\setlength{\evensidemargin}{-0.25in}
%\setlength{\headsep}{10pt}

%Use changebar.sty  to track changes.

%Saving space: see
%   http://www-h.eng.cam.ac.uk/help/tpl/textprocessing/squeeze.html

%Page layout info:
%   http://amath.colorado.edu/documentation/LaTeX/reference/layout.html



%Latex
%\documentstyle[fleqn,psfig,epsfig]{article}
%\documentstyle[psfig]{article}
%\setlength{\textwidth}{6.5in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\textheight}{8.5in}
%\setlength{\headheight}{0in}
%\setlength{\headsep}{0in}
%\setlength{\parindent}{0in} % block style
%\setlength{\parskip}{0.3cm}

\newtheorem{thm}{Theorem}[section]
\newtheorem{corr}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}
\newenvironment{myproof}{{\bf Proof.}}{}
\newtheorem{prop}{Proposition}[section]

\newcommand{\intersect}{\mbox{$\cap$}}
%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\mbox{$\frac{1}{2}$}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
%\newcommand{\defeq}{\mbox{$\stackrel{\rm def}{=}}$}
%\newcommand{\real}{{\rm I\hspace{-0.2em}R}}
\newcommand{\real}{\mbox{$\mathbb{R}$}}
\newcommand{\indep}{\mbox{$\perp$}}
\newcommand{\given}{\mbox{$|$}}
\newcommand{\ra}{\mbox{$\rightarrow$}}
\newcommand{\lra}{\mbox{$\leftrightarrow$}}
\newcommand{\Ra}{\mbox{$\Rightarrow$}}
\newcommand{\la}{\mbox{$\leftarrow$}}
\newcommand{\tr}{\mbox{$\mbox{tr}$}}
%\newcommand{\det}{\mbox{$\mbox{det}$}}

\newcommand{\rnd}[1]{\left(#1\right)}
\newcommand{\sqr}[1]{\left[#1\right]}
\newcommand{\crl}[1]{\left\{#1\right\}}
\newcommand{\ang}[1]{\langle#1\right\rangle}
\newcommand{\myexpect}{\mathbb{E}}


\newcommand{\range}{\mbox{$\mbox{range}$}} 
\newcommand{\myspan}{\mbox{$\mbox{span}$}}
\newcommand{\nullspace}{\mbox{$\mbox{nullspace}$}}
\newcommand{\adj}{\mbox{$\mbox{adj}$}}
\newcommand{\nbd}{\mbox{$\mbox{nbd}$}}





\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\mbox{Discrete}}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{\mbox{${\cal N}$}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{\mbox{$NI\chi^2$}}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{\mbox{$p$}}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{\mbox{${\cal T}$}}
\newcommand{\student}{\mbox{${\cal T}$}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}


\newcommand{\define}[1]{{\bf #1}}

\newcommand{\solnsrc}[1]{Source: #1}
\newcommand{\exsrc}[1]{(Source: #1)}

%\newenvironment{nam}[args]{begdef}{enddef}
%\newcommand{\includecodefig}[3]{
%\begin{figure}
%\noindent
%\hrulefill  
%\verbatiminput{#1}
%\noindent
%\hrulefill
%\noindent 
%}
%\caption{#2}
%\label{#3}
%\end{figure}
%}







%\newcommand{\includedudafig}[3]{
%\begin{figure}
%\centerline{\epsfig{file=c:/kmurphy/figures/duda/duda-#1.eps,height=#2}}
%\caption{#3 Source:
%\protect\cite{Duda01} Fig #1.}
%%Fig #1.}
%\label{fig:duda#1}
%\end{figure}
%}


%\newcommand{\keyword}[1]{{\bf #1}}
\newcommand{\keyword}[1]{{\bf #1}\index{keywords}{#1}}
\newcommand{\addtoindex}[1]{#1 \index{keywords}{#1}}
\newcommand{\keywordSpecial}[2]{{\bf #1}\index{keywords}{#2@#1}}
\newcommand{\bfidx}[1]{{\bf #1}}
\newcommand{\keywordDef}[1]{{\bf #1}\index{keywords}{#1|bfidx}}
%\newcommand{\keyworddef}[1]{{\bf #1}\index{keywords}{#1@{\bf #1}}}
\newcommand{\codename}[1]{{\tt #1}\index{code}{#1}}
\newcommand{\netlabname}[1]{{\tt #1}}
\newcommand{\Rcmd}[1]{{\tt #1}}
\newcommand{\matlabcmd}[1]{{\tt #1}}
\newcommand{\matlabscript}[1]{{\tt #1}}
\newcommand{\dataname}[1]{{\tt #1}}

%\newcommand{\dim}{\mbox{dim}}
\newcommand{\softmax}{\calS}
%\newcommand{\softmax}{\mbox{softmax}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\MLABA}{\mbox{FML}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\myvec}[1]{\mbox{$\mathbf{#1}$}}
\newcommand{\myvecsym}[1]{\mbox{$\boldsymbol{#1}$}}

\newcommand{\vzero}{\mbox{$\myvecsym{0}$}}
\newcommand{\vone}{\mbox{$\myvecsym{1}$}}

\newcommand{\valpha}{\mbox{$\myvecsym{\alpha}$}}
\newcommand{\vbeta}{\mbox{$\myvecsym{\beta}$}}
\newcommand{\vchi}{\mbox{$\myvecsym{\chi}$}}
\newcommand{\vdelta}{\mbox{$\myvecsym{\delta}$}}
\newcommand{\vDelta}{\mbox{$\myvecsym{\Delta}$}}
\newcommand{\vepsilon}{\mbox{$\myvecsym{\epsilon}$}}
\newcommand{\veta}{\mbox{$\myvecsym{\eta}$}}
\newcommand{\vgamma}{\mbox{$\myvecsym{\gamma}$}}
\newcommand{\vmu}{\mbox{$\myvecsym{\mu}$}}
\newcommand{\vlambda}{\mbox{$\myvecsym{\lambda}$}}
\newcommand{\vLambda}{\mbox{$\myvecsym{\Lambda}$}}
\newcommand{\vLambdaBar}{\mbox{$\overline{\vLambda}$}}
\newcommand{\vrho}{\mbox{$\myvecsym{\rho}$}}
\newcommand{\vphi}{\mbox{$\myvecsym{\phi}$}}
\newcommand{\vPhi}{\mbox{$\myvecsym{\Phi}$}}
\newcommand{\vpi}{\mbox{$\myvecsym{\pi}$}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\mbox{$\myvecsym{\Psi}$}}
\newcommand{\vtheta}{\mbox{$\myvecsym{\theta}$}}
\newcommand{\vTheta}{\mbox{$\myvecsym{\Theta}$}}
\newcommand{\vsigma}{\mbox{$\myvecsym{\sigma}$}}
\newcommand{\vSigma}{\mbox{$\myvecsym{\Sigma}$}}
\newcommand{\vOmega}{\mbox{$\myvecsym{\Omega}$}}
\newcommand{\vtau}{\mbox{$\myvecsym{\tau}$}}
\newcommand{\vxi}{\mbox{$\myvecsym{\xi}$}}
\newcommand{\vvarepsilon}{\mbox{$\myvecsym{\varepsilon}$}}

\newcommand{\va}{\mbox{$\myvec{a}$}}
\newcommand{\vb}{\mbox{$\myvec{b}$}}
\newcommand{\vc}{\mbox{$\myvec{c}$}}
\newcommand{\vd}{\mbox{$\myvec{d}$}}
\newcommand{\ve}{\mbox{$\myvec{e}$}}
\newcommand{\vf}{\mbox{$\myvec{f}$}}
\newcommand{\vg}{\mbox{$\myvec{g}$}}
\newcommand{\vh}{\mbox{$\myvec{h}$}}
\newcommand{\vj}{\mbox{$\myvec{j}$}}
\newcommand{\vk}{\mbox{$\myvec{k}$}}
\newcommand{\vm}{\mbox{$\myvec{m}$}}
\newcommand{\vn}{\mbox{$\myvec{n}$}}
\newcommand{\vp}{\mbox{$\myvec{p}$}}
\newcommand{\vq}{\mbox{$\myvec{q}$}}
\newcommand{\vr}{\mbox{$\myvec{r}$}}
\newcommand{\vs}{\mbox{$\myvec{s}$}}
\newcommand{\vt}{\mbox{$\myvec{t}$}}
\newcommand{\vu}{\mbox{$\myvec{u}$}}
\newcommand{\vv}{\mbox{$\myvec{v}$}}
\newcommand{\vw}{\mbox{$\myvec{w}$}}
\newcommand{\vws}{\mbox{$\vw_s$}}
\newcommand{\vwh}{\mbox{$\hat{\vw}$}}
\newcommand{\vx}{\mbox{$\myvec{x}$}}
\newcommand{\vxt}{\mbox{$\myvec{\tilde{x}}$}}
\newcommand{\vy}{\mbox{$\myvec{y}$}}
\newcommand{\vyt}{\mbox{$\myvec{\tilde{y}}$}}
\newcommand{\vz}{\mbox{$\myvec{z}$}}

\newcommand{\vA}{\mbox{$\myvec{A}$}}
\newcommand{\vB}{\mbox{$\myvec{B}$}}
\newcommand{\vC}{\mbox{$\myvec{C}$}}
\newcommand{\vD}{\mbox{$\myvec{D}$}}
\newcommand{\vE}{\mbox{$\myvec{E}$}}
\newcommand{\vF}{\mbox{$\myvec{F}$}}
\newcommand{\vG}{\mbox{$\myvec{G}$}}
\newcommand{\vH}{\mbox{$\myvec{H}$}}
\newcommand{\vI}{\mbox{$\myvec{I}$}}
\newcommand{\vJ}{\mbox{$\myvec{J}$}}
\newcommand{\vK}{\mbox{$\myvec{K}$}}
\newcommand{\vL}{\mbox{$\myvec{L}$}}
\newcommand{\vM}{\mbox{$\myvec{M}$}}
\newcommand{\vN}{\mbox{$\myvec{N}$}}
\newcommand{\vO}{\mbox{$\myvec{O}$}}
\newcommand{\vP}{\mbox{$\myvec{P}$}}
\newcommand{\vQ}{\mbox{$\myvec{Q}$}}
\newcommand{\vR}{\mbox{$\myvec{R}$}}
\newcommand{\vS}{\mbox{$\myvec{S}$}}
\newcommand{\vT}{\mbox{$\myvec{T}$}}
\newcommand{\vU}{\mbox{$\myvec{U}$}}
\newcommand{\vV}{\mbox{$\myvec{V}$}}
\newcommand{\vW}{\mbox{$\myvec{W}$}}
\newcommand{\vX}{\mbox{$\myvec{X}$}}
%\newcommand{\vXs}{\mbox{$\vX_{\vs}$}}
\newcommand{\vXs}{\mbox{$\vX_{s}$}}
\newcommand{\vXt}{\mbox{$\myvec{\tilde{X}}$}}
\newcommand{\vY}{\mbox{$\myvec{Y}$}}
\newcommand{\vZ}{\mbox{$\myvec{Z}$}}


\newcommand{\vxtest}{\mbox{$\myvec{x}_*$}}
\newcommand{\vytest}{\mbox{$\myvec{y}_*$}}


%\newcommand{\matlab}{{\bf MATLAB exercise}}
\newcommand{\matlabex}{(Matlab)}
%\newcommand{\matlabexx}{{\bf MATLAB exercise}\\}
\newcommand{\matlabexx}{}

\newcommand{\ftrue}{\mbox{$f_{true}$}}

\newcommand{\precw}{\mbox{$\lambda_{w}$}} % precision of weights (alpha)
\newcommand{\precy}{\mbox{$\lambda_{y}$}} % precision of y (beta)
\newcommand{\fbar}{\mbox{$\overline{f}$}}
\newcommand{\xbar}{\mbox{$\overline{x}$}}
\newcommand{\ybar}{\mbox{$\overline{y}$}}
\newcommand{\vxbar}{\mbox{$\overline{\vx}$}}
\newcommand{\vybar}{\mbox{$\overline{\vy}$}}
\newcommand{\Xbar}{\mbox{$\overline{X}$}}
\newcommand{\Ybar}{\mbox{$\overline{Y}$}}
\newcommand{\Jbar}{\mbox{$\overline{J}$}}
\newcommand{\Lbar}{\mbox{$\overline{L}$}}
\newcommand{\Tbar}{\mbox{$\overline{T}$}}

\newcommand{\htilde}{\mbox{$\tilde{h}$}}
\newcommand{\vhtilde}{\mbox{$\tilde{\vh}$}}
\newcommand{\Dtilde}{\mbox{$\tilde{D}$}}
\newcommand{\wtilde}{\mbox{$\tilde{w}$}}
\newcommand{\xtilde}{\mbox{$\tilde{x}$}}
\newcommand{\Xtilde}{\mbox{$\tilde{X}$}}
\newcommand{\ytilde}{\mbox{$\tilde{y}$}}
\newcommand{\Ytilde}{\mbox{$\tilde{Y}$}}
\newcommand{\vxtilde}{\mbox{$\tilde{\vx}$}}
\newcommand{\vytilde}{\mbox{$\tilde{\vy}$}}
\newcommand{\ztilde}{\mbox{$\tilde{\z}$}}
\newcommand{\vztilde}{\mbox{$\tilde{\vz}$}}
\newcommand{\vthetaMAP}{\mbox{$\hat{\vtheta}_{MAP}$}}
\newcommand{\vthetahat}{\mbox{$\hat{\vtheta}$}}
\newcommand{\thetahat}{\mbox{$\hat{\theta}$}}
\newcommand{\thetabar}{\mbox{$\overline{\theta}$}}
\newcommand{\vthetabar}{\mbox{$\overline{\vtheta}$}}
\newcommand{\pibar}{\mbox{$\overline{\pi}$}}
\newcommand{\vpibar}{\mbox{$\overline{\vpi}$}}



\newcommand{\sss}{\mbox{$s^2$}}
\newcommand{\vvv}{\mbox{$v$}}
\newcommand{\RSS}{\mbox{RSS}}

%\newcommand{\do}{\mbox{$\mbox{do}$}}


\newcommand{\vvec}{\mbox{$\mbox{vec}$}}
\newcommand{\dof}{\mbox{$\mbox{dof}$}}
\newcommand{\E}{\mbox{$E \;$}}
\newcommand{\Var}{\mbox{$\mbox{Var} \;$}}
\newcommand{\Std}{\mbox{$\mbox{Std} \;$}}
\newcommand{\Vvar}{\mbox{$\mbox{Var}$}}
%\newcommand{\mean}{\mbox{$\mbox{mean} \;$}}
%\newcommand{\mmean}{\mbox{$\mbox{mean}$}}
\newcommand{\mode}{\mbox{$\mbox{Mode} \;$}}
\newcommand{\Mode}{\mbox{$\mbox{Mode} \;$}}
\newcommand{\Mmode}{\mbox{$\mbox{Mode}$}}
\newcommand{\Cov}{\mbox{$\mbox{Cov}$}}
%\newcommand{\diag}{\mbox{$\mbox{diag}$}}
\newcommand{\diag}{\mbox{$\mbox{diag}$}}
\newcommand{\bias}{\mbox{$\mbox{bias}$}}
%\newcommand{\dim}{\mbox{$\mbox{dim}$}}
%\newcommand{\intersect}{\mbox{$\cap$}}
\newcommand{\union}{\mbox{$\cup$}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{Tr}}


\newcommand{\NN}{\mbox{$N$}}
\newcommand{\NC}{\mbox{$N_C$}}
\newcommand{\ND}{\mbox{$N_D$}}
\newcommand{\NX}{\mbox{$N_X$}}
\newcommand{\NXi}{\mbox{$N_{X_i}$}}
\newcommand{\NY}{\mbox{$N_Y$}}

\newcommand{\nx}{\mbox{$n_x$}}
\newcommand{\ny}{\mbox{$n_y$}}
\newcommand{\nv}{\mbox{$n_v$}}
\newcommand{\nk}{\mbox{$n_k$}}
\newcommand{\nn}{\mbox{$n$}}

%\newcommand{\xdi}{\mbox{$x_{di}$}}
%\newcommand{\xji}{\mbox{$x_{ji}$}}
%\newcommand{\yi}{\mbox{$y_i$}}



\newcommand{\ki}{i}
\newcommand{\kj}{j}
\newcommand{\kk}{k}

\newcommand{\kC}{C}
\newcommand{\kc}{c}
\newcommand{\calA}{\mbox{${\cal A}$}}
\newcommand{\calB}{\mbox{${\cal B}$}}
\newcommand{\calC}{\mbox{${\cal C}$}}
\newcommand{\calD}{\mbox{${\cal D}$}}
\newcommand{\calDx}{\mbox{${\cal D}_x$}}
\newcommand{\calE}{\mbox{${\cal E}$}}
\newcommand{\calF}{\mbox{${\cal F}$}}
\newcommand{\calG}{\mbox{${\cal G}$}}
\newcommand{\calH}{\mbox{${\cal H}$}}
\newcommand{\calHX}{\mbox{${\cal H}_X$}}
\newcommand{\calHy}{\mbox{${\cal H}_y$}}
\newcommand{\calI}{\mbox{${\cal I}$}}
\newcommand{\calK}{\mbox{${\cal K}$}}
\newcommand{\calM}{\mbox{${\cal M}$}}
\newcommand{\calMp}{\mbox{$\calM^+$}}
\newcommand{\calMm}{\mbox{$\calM^-$}}
\newcommand{\calMo}{\mbox{$\calM^o$}}
\newcommand{\Ctest}{\mbox{$C_*$}}
\newcommand{\calP}{\mbox{${\cal P}$}}
\newcommand{\calS}{\mbox{${\cal S}$}}
\newcommand{\calSstar}{\mbox{$\calS_*$}}
\newcommand{\calT}{\mbox{${\cal T}$}}
\newcommand{\calV}{\mbox{${\cal V}$}}
\newcommand{\calX}{\mbox{${\cal X}$}}
\newcommand{\calY}{\mbox{${\cal Y}$}}

\newcommand{\score}{\mbox{$\mbox{score}$}}
\newcommand{\scoreBIC}{\mbox{$\mbox{score-BIC}$}}
\newcommand{\scoreBICL}{\mbox{$\mbox{score-BIC-L1}$}}
\newcommand{\scoreL}{\mbox{$\mbox{score-L1}$}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{$\mbox{do}$}}
\newcommand{\data}{\calD}
\newcommand{\futuredata}{\tilde{\calD}}
%\newcommand{\data}{\mbox{$D$}}
\newcommand{\costfunc}{\mathcal{L}}
\newcommand{\err}{\mbox{$\mbox{errr}$}}
\newcommand{\logit}{\mbox{$\mbox{logit}$}}
\newcommand{\probit}{\mbox{$\mbox{probit}$}}
\newcommand{\sigmoid}{\mbox{$\sigma$}}

% We want to avoid name clashes with the exercise.sty package
%\newenvironment{myexercises}{\section{Exercises}}{}
\newenvironment{myexercises}{\section{Exercises}}{}
%\newenvironment{solutions}{\section*{Solutions} \begin{solutionsTag}}{\end{solutionsTag}}
%\newenvironment{solutions}{\section*{Solutions} \begin{comment}}{\end{comment}}
\newenvironment{mysolutions}{\section{Solutions}}{}
\newcommand{\myexercise}[1]{\vspace{0.5cm} \subsection{#1}}
\newcommand{\mysoln}[1]{\vspace{0.5cm} \subsection{#1}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

%skip numbering the equation
\newcommand{\numberthis}{\addtocounter{equation}{1}\tag{\theequation}}

\usepackage{amsmath}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%zero one noise
\newcommand{\gnoise}{\mathcal{N}(0,\sigma^2)}
